Robust Analysis of Auction Equilibria

Equilibria in auctions can be very difficult to analyze, beyond the symmetric environments where revenue equivalence renders the analysis straightforward. This paper takes a robust approach to evaluating the equilibria of auctions. Rather than identify the equilibria of an auction under specific environmental conditions, it considers worst-case analysis, where an auction is evaluated according to the worst environment and worst equilibrium in that environment. It identifies a non-equilibrium property of auctions that governs whether or not their worst-case equilibria are good for welfare and revenue. This property is easy to analyze, can be refined from data, and composes across markets where multiple auctions are run simultaneously.

==> beyondwpb-ap.tex <==
\subsection{All-Pay Mechanisms}
\label{sec:allpay}

In this section, we use our generalized framework to derive robust welfare guarantees for all-pay mechanisms. Agents in an all-pay mechanism directly manage their tradeoff between allocation and payments via their bid. We show in Section~\ref{sec:apreduction} that when allocation requires a high bid, this translates to a high price per unit of allocation.   This implies generalized \rc\ guarantees for the all-pay implementations of the allocation rules studied in Section~\ref{sec:rc}. In Section~\ref{sec:native}, we improve our welfare guarantees using an alternative, all-pay specific formulation of \trc. Our alternative formulation forgoes the translation from all-pay bid to price per unit of allocation.

\subsubsection{Reduction to Winner-Pays-Bid Analysis}
\label{sec:apreduction}

For a feasibility environment $\feasible$ and bid allocation rule $\bidalloc$, the all-pay mechanism for $\bidalloc$ solicits a bid $\bidagent$ from each agent, selects winners according to $\bidalloc(\bids)$, and charges each agent their bid. Hence, the revenue of an all-pay mechanism is the sum of all bids, which is at least the bids of just the winners, as in a winner-pays-bid mechanism. Fixing a distribution of bids, though, note that agents' threshold bids are independent of the payment rule. To characterize the \rc\ of all-pay mechanisms, we will therefore relate revenue to agents' threshold bids using the winner-pays-bid analysis of Section~\ref{sec:rc}, and then relate each agent's threshold bid to their threshold price per unit. In other words, we will reduce the analysis of all-pay mechanisms to that of winner-pays-bid mechanisms. We will consider only deterministic feasibility environments and mechanisms, with allocations in $\{0,1\}^{\numagents}$. Our alternative \rc\ formulation in the next section will relax this requirement.

\textcolor{red}{SWITCH TO BIDS B RATHER THAN ACTIONS A}

By Corollary~\ref{cor:gendegen}, it suffices to analyze the generalized \rc\ on degenerate priors, so we omit conditioning on $\valagent$. Consider a bid profile $\bids$, i.e.\ a strategy profile for a degenerate prior. When the mechanism and environment are both deterministic, the generalized threshold surplus for every agent simplifies to their threshold bid $\thresholdagent(\bidothers)=\inf\{\bidagent\,|\,\bidallocagent(\bidagent,\bidothers)
= 1\}$.

\begin{lemma}
	Let $\mech$ be a deterministic mechanism for a deterministic allocation environment $\feasible$. Then for any (implicit) degenerate prior and bid profile $\bids$, $\equivcumulative{\agent}{1}{}  =\thresholdagent(\bidothers)$.
\end{lemma}
\begin{proof}
	For any bid $\bid< \thresholdagent(\bidothers)$, the price per unit $\equivbidact{b}$ for $b$ is infinite, as $\bidallocagent(b,\bidothers)=0$. For $\bid\geq \thresholdagent(\bidothers)$, the price per unit is $\bid$, as $\agent$ is allocated with probability $1$. It follows that for any $z\in(0,1]$, $\equivthresh{\agent}{z}=\inf_{b\,:\,\bidallocagent(b)\geq z} \equivbidact{b}=\thresholdagent(\bidothers)$. From the definition of threshold surplus, we therefore obtain $\equivcumulative{\agent}{1}{}=\int_0^{1}\equivthreshres{\agent}{\allocation}{}\,d\allocation=\thresholdagent(\bidothers)$.
\end{proof}

\textcolor{red}{Stopped here}

 for an agent $\agent$ is simply their threshold bid $\thresholdagent(\bidothers)=\inf\{\bidagent\,|\,\bidallocagent(\bidagent,\bidothers)
= 1\}$.

%old
% Formally, given a strategy profile $\strat$ for a degenerate prior, i.e.\ an action profile $\actions$, recall the notation for threshold bids from Section~\ref{sec:rc}. We denote by $\interthresh{i}{\allocation}=\inf \{\bid\,|\,\bidallocagent(\bid)\geq \allocation\}$ agent $\agent$'s threshold bid for allocation level $\allocation$, and $\cumuthreshagent{\agent}{\allocation}{}=\int_0^{\allocation}\interthreshres{\agent}{z}{}\,dz$ their cumulative threshold for $\allocation$. We consider mechanisms without reserves, as is conventional for all-pay mechanisms. Note that $\interthresh{i}{\allocation}$ and $\cumuthreshagent{\agent}{\allocation}{}$ are only a property of the bid-allocation rule being used, and not the payment rule. Hence, all-pay mechanisms inherit the approximation relationships observed in our study of winner-pays-bid mechanisms. Formally:

\begin{lemma}\label{lem:aprc}
	Let $\mech$ and $\mech'$ be all-pay and winner-pays-bid mechanisms with allocation rule $\bidalloc$. If $\mech'$ has \rc\ $\revpar$, then for any action profile $\actions$, and feasible allocation $\allocalt$:
	\begin{equation*}
	\rev(\mech,\actions)\geq\tfrac{1}{\revpar}\sum\nolimits_{\agent}\cumuthreshagent{\agent}{\allocaltagent}{}.
	\end{equation*}
\end{lemma}
\begin{proof}
	A winner-pays-bid mechanism $\mech'$ has \rc\ $\revpar$ only if
	\begin{equation*}
	\rev(\mech',\actions)\geq\tfrac{1}{\revpar}\sum\nolimits_{\agent}\cumuthreshagent{\agent}{\allocaltagent}{}.
	\end{equation*}
	The lemma follows from noting that for the same action profile, $\rev(\mech,\actions)\geq \rev(\mech',\actions)$, as an all-pay auction charges all agents their bid, rather than just the winners.
\end{proof}

A generalized \rc\ result will follow from relating the bidspace threshold surpluses $\cumuthreshagent{\agent}{\cdot}{}$ to the generalized versions $\equivcumulative{\agent}{\cdot}{}$.

\begin{lemma}\label{lem:chebyshev}
	For any action profile $\actions$ and agent $\agent$, $2\cumuthreshagent{\agent}{1}{}\geq \equivcumulative{\agent}{1}{}$.
\end{lemma}

\begin{proof}
	For any bid $\bidagent$ in an all-pay auction, the price per unit is given by $\equivbid(\bidagent)=\bidagent/\bidallocagent(\bidagent)$. Hence, threshold bids and threshold price per units are related as $\equivthresh{\agent}{z}=\interthresh{i}{z}/z$.
	Hence, by Chebyshev's sum inequality, we have:
	\begin{equation*}
	\cumuthreshagent{\agent}{1}{}=\int_0^{1}\interthresh{i}{z}\,dz\geq \frac{1}{2}\int_0^{1}\equivthresh{\agent}{z}\,dz= \frac{\equivcumulative{\agent}{1}{}}{2}.\qedhere
	\end{equation*}
\end{proof}
By combining Lemmas~\ref{lem:aprc} and~\ref{lem:chebyshev}, we observe that determinsitic all-pay mechansisms inherit \rc\ guarantees from their first-price counterparts.

\begin{theorem}\label{thm:apweak}
	Let $\mech$ and $\mech'$ be all-pay and winner-pays-bid mechanisms with allocation rule $\bidalloc:\mathbb R^{\numagents}\rightarrow \{0,1\}^{\numagents}$. If $\mech'$ has \rc\ $\revpar$, then $\mech$ has generalized \rc\ $2\revpar$.
\end{theorem}

\begin{proof}
	Let $\actionsdist$ be a distribution of bids, and $\allocalt$ be a feasible allocation. By Lemma~\ref{lem:aprc}, we have: $\rev(\mech,\actionsdist)\geq\tfrac{1}{\revpar}\sum\nolimits_{\agent}\cumuthreshagent{\agent}{\allocaltagent}{}$. Since $\allocaltagent\in\{0,1\}$ for all agents $\agent$, Lemma~\ref{lem:chebyshev} implies $\tfrac{1}{\revpar}\sum\nolimits_{\agent}\cumuthreshagent{\agent}{\allocaltagent}{}\geq \tfrac{1}{2\revpar}\sum\nolimits_{\agent}\equivcumulative{\agent}{\allocaltagent}{}$, proving the theorem.
\end{proof}


\subsubsection{All-Pay Native Framework}
\label{sec:native}

The generalized \rc\ studies the extent to which competition, measured by threshold price per unit of allocation, is captured by a mechanism as revenue. Agents' utilities trade off with their threshold price per unit, which implies robust welfare and revenue guarantees. The bidding problem in all-pay mechanisms suggests another, equivalent tradeoff inherent in best response, between agents' utility and their threshold {\em payments}. In this section, we use this intuition to guide an alternative formulation of \trc. This will improve the guarantees of the previous section in two senses. First, it will produce better worst-case approximation ratios. Second, it will apply to randomized as well as deterministic mechanisms.

As in the previous section, denote by $\interthresh{i}{\allocation}$ agent $\agent$'s interim threshold bid, and $\cumuthreshagent{\agent}{\allocation}{}$ their threshold surplus. We will study the relationship between these quantities and revenue.

\begin{definition}\label{def:aprc}
	Given an all-pay mechanism $\mech$, we say $\mech$ has all-pay \rc\ $\revpar$ if for any distribution of bids $\actionsdist$ and feasible allocation $\allocalt$, we have:
	\begin{equation*}
	\rev(\mech,\actionsdist)\geq \tfrac{1}{\revpar}\sum\nolimits_{\agent}\cumuthreshagent{\agent}{\allocalt}{}.
	\end{equation*}
\end{definition}
As an immediate corollary of Lemma~\ref{lem:aprc}, we have:
\begin{corollary}
	Let $\mech$ and $\mech'$ be all-pay and winner-pays-bid mechanisms with allocation rule $\bidalloc$. If $\mech'$ has \rc\ $\revpar$, then $\mech$ has all-pay \rc\ $\revpar$.
\end{corollary}

Definition~\ref{def:aprc} allows us to reason directly about agents' bidding problem in all-pay mechanisms. The appropriate analog of individual efficiency becomes:
\begin{lemma}\label{lem:aptradeoff}
	Let $\bidallocation$ be a single-agent allocation rule mapping bids to allocations. Let $\bid(\cdot)$ be a function mapping values to best response bids under $\bidallocation$ with all-pay payments. Then for every value $\val$ and $z\in[0,1]$:
	\begin{equation*}
	\bidutil(\bid(\val))+\cumuthresh(z)\geq \tfrac{1}{2}\val z.
	\end{equation*}
\end{lemma}
\begin{proof}
	The proof follows that of Lemma~\ref{lem:brres}. The agent selects their best response bid $\bid$ to maximize their utility $\bidutil(\bid)=\val\bidallocation(\bid)-\bid$. For any allocation probability $\allocation\in[0,1]$, agent $\agent$ could choose to get allocation probability at least $\allocation$ by bidding their interim threshold $\interthresh{}{\allocation}$. Hence, $\bidutil(
	\bid(\val))\geq \val \allocation-\interthresh{}{\allocation}$ for all $\allocation\in[0,1]$. We may rearrange this as $\interthresh{}{\allocation}\geq \val\allocation-\bidutil(\bid(\val))$. Since we also have $\interthresh{}{\allocation}\geq 0$, we may write:
	\begin{align*}
	\cumuthreshagent{}{z}{}\geq \int_0^z \max(\val\allocation-\bidutil(\bid(\val)),0)\,d\allocation&=\int_{\bidutil(\bid(\val))/\val}^z \val\allocation-\bidutil(\bid(\val))\,d\allocation\\
	&=\tfrac{\val}{2}-\bidutil(\bid(\val))+\tfrac{\bidutil(\bid(\val))^2}{2\val}.
	\end{align*}
	We therefore have $\bidutil(\bid(\val))+\cumuthreshagent{}{z}{}\geq \val/2+\bidutil(\val)^2/2\val$. Holding $\val$ fixed and minimizing the righthand side as a function of $\bidutil(\bid(\val))$ yields a lower bound of $\val z/2$, as desired.
\end{proof}

Aggregating Lemma~\ref{lem:aptradeoff} yields robust welfare guarantee. The proof is mechanically identical to that of Theorem~\ref{thm:restowelf}.

\begin{theorem}\label{thm:apstrong}
Any mechanism with all-pay \rc\ $\revpar\geq1$ has worst-case welfare approximation $2\revpar$ in Bayes-Nash equilibrium.
\end{theorem}

Theorem~\ref{thm:apstrong} yields stronger guarantees than Theorem~\ref{thm:apweak}. For instance, for the single-item all-pay auction, Theorem~\ref{thm:apweak} implies a worst-case welfare approximation of $2e/(e-1)$, compared to the $2$ derived from Theorem~\ref{thm:apstrong}. Moreover, we obtain an approximation of $2$ for position auctions, which did not follow from Theorem~\ref{thm:apweak}.



==> dhnotation.tex <==
\newcommand{\restate}[2]{\vspace{0.1in} \noindent{\bf #1 (Restatement).}
{\em #2} }



\newcommand{\rank}{y}
\newcommand{\rankagent}{\rank_{\agent}}

\newcommand{\allocgroup}{\allocation_{j}}
%\newcommand{\bidcdf}{B}
\newcommand{\bidcdfothers}{\bidcdf_{-i}}

==> generalres.tex <==
\subsection{Resolution of Generalized Revenue Covering}
\label{sec:genres}

In winner-pays-bid mechanisms, an agent's best response problem is one of explicitly trading off allocation probability against price per unit of allocation, measured by their bid. The resolution bounds of Section~\ref{sec:resolution} followed from quantifying this tradeoff. As we have defined thresholds prices for general mechanisms in terms of price per unit of allocation, identical bounds will follow from a similar analysis. As in Section~\ref{sec:resolution}, we assume $\revpar\geq 1$. This will hold for all mechanisms we study. We begin with the objective of Bayes-Nash welfare. An agent either obtains high utility from winning or must pay a high price per unit of allocation:



\begin{proof}
Agent $\agent$ selects an action $\actionagent$ which maximizes their expected utility $\bidutilagent(\actionagent)=\valagent\bidallocagent(\actionagent)-\bidpaymentagent(\actionagent)$. Their utility is lower bounded by the utility they would obtain by securing allocation probability $\allocation$ with the minimum price per unit. Hence, $\utilagent(\valagent)\geq (\valagent -\equivthresh{\agent}{\allocation})\allocation$.
%	 \begin{equation*}
%	 \utilagent(\valagent)\geq \valagent\bidallocagent(\induceact(\allocation))-\bidpaymentagent(\induceact(\allocation))=(\valagent-\equivthresh{\agent}{\allocation})\bidallocagent(\induceact(\allocation)).
%	 \end{equation*}
	 This implies a lower bound on $\equivthresh{\agent}{\allocation}$: $\equivthresh{\agent}{\allocation}
	 %\geq\valagent-\utilagent(\valagent)/\bidallocagent(\induceact(\allocation))
	 \geq \valagent-\utilagent(\valagent)/\allocation$. By definition,  $\equivthresh{\agent}{\allocation}\geq 0$ as well. Integrating these two lower bounds yields
	 \begin{equation*}
	 \equivcumulative{\agent}{z}{}\geq \int_0^z \max(\valagent-\tfrac{\utilagent(\valagent)}{\allocation},0)\,d\allocation,= z-\utilagent(\valagent)(1-\ln\tfrac{\utilagent(\valagent)}{\valagent z}).
	 \end{equation*}
	 	Hence, $\utilagent(\valagent)+\equivcumulative{\agent}{z}{}\geq \valagent z -\utilagent(\valagent)\ln(\utilagent(\valagent)/\valagent z)$. Holding $\valagent$ fixed and minimizing the righthand side as a function of $\utilagent(\valagent)$ yields the lower bound $\valagent z(e-1)/e$.
\end{proof}

The tradeoff of Lemma~\ref{lem:genweltradeoff} may be aggregated exactly as in the proof of Theorem~\ref{thm:welfare-bne} to obtain the following bound on resolution:

\begin{theorem}
	The resolution of generalized revenue covering for Bayes-Nash equilibrium and the objective of welfare is at most $e/(e-1)$.
\end{theorem}

A bound on resolution for revenue in BNE follows from an analysis similar to that of Section~\ref{sec:welfare-bnerev}. We will restrict attention to mechanisms where any action $\actionagent$ for agent $\agent$ with $\bidallocagent(\actionagent)>0$ must also have minimum price per unit $\equivbidact{\actionagent}\geq \reserveagentm$, where $\reserveagentm$ is $\agent$'s monopoly reserve. Such mechanisms exclude agents with value $\valagent<\reserveagentm$ in equilibrium, since any bid which secures positive allocation also has negative utility. Moreover, agents who do win must do so at a high price per unit. Winner-pays-bid mechanisms with monopoly reserves clearly satisfy this condition, as agents with value $\valagent<\reserveagentm$ will not overbid. Similar reasoning will apply to simultaneous winner-pays-bid mechanisms, which we define formally in Section~\ref{sec:simultaneous}. 

To prove our bound, we first derive a tradeoff between an agent's contribution to virtual surplus and their competition:

\begin{lemma}\label{lem:genrevtradeoff}
	Let $\strat$ be a Bayes-Nash equilibrium of a mechanism, and let $\agent$ be an agent with value $\valagent$ satisfying $\vvalagent(\valagent)\geq 0$  and $\valagent\geq \reserveagentm$. Further assume that for any action $\actionagent$ with $\bidallocagent(\actionagent)>0$, $\equivbidact{\actionagent}\geq \reserveagentm$. Then for any $z\in [0,1]$, we have:
	\begin{equation}\label{eq:genvvalcover}
	\vvalagent(\valagent)\allocagent(\valagent)+\equivcumulative{\agent}{z}{\reserveagentm}\geq \tfrac{e-1}{e}\vvalagent(\valagent) z.
	\end{equation}
\end{lemma}

\begin{proof}
	\newcommand{\topallocagent}{\overline \allocation_{\agent}}
	
	Our proof generalizes that of Lemma~\ref{lem:revtradeoff}. Let $\agent$ be an agent with realized value $\valagent\geq \reserveagentm$ and nonnegative virtual value $\vvalagent(\valagent)\geq 0$. Define $\topallocagent=\sup \{ z\,|\equivthresh{\agent}{z}\leq \reserveagentm\}$ to be the largest allocation attainable at price per unit at most $\reserveagentm$. We begin by lowerbounding $\agent$'s equilibrium payments as $\paymentagent(\valagent)\geq \reserveagentm\topallocagent$ by considering two cases. First, if there is an action $\actionagent$ which in equilibrium satisfies $\equivbidact{\actionagent}\leq \valagent$ and $\bidallocagent(\action)>0$, then the action taken by $\agent$, $\stratagent(\valagent)$, will be such an action. In this case, $\paymentagent(\valagent)=\equivbidagent(\stratagent(\valagent))\allocagent(\valagent)\geq \reserveagentm\topallocagent$. Otherwise, all actions with positive allocation have price per unit at least $\valagent$, and hence at least $\reserveagentm$. In this case, $\topallocagent=0$, and the desired inequality holds trivially.
	
	Next, note that by the definition of $\topallocagent$,
	\begin{equation*}
	\equivcumulative{\agent}{z}{}-\equivcumulative{\agent}{z}{\reserveagentm}=\int_0^{\topallocagent}\equivthresh{\agent}{z}\,dz\leq \reserveagent\topallocagent.
	\end{equation*}
	Combining these facts with Lemma~\ref{lem:genweltradeoff} yields:
\begin{equation}\label{eq:genvvalcoverres}
\valagent\allocagent(\valagent)+\equivcumulative{\agent}{z}{\reserveagentm}= \utilagent(\valagent)+\paymentagent(\valagent)+\equivcumulative{\agent}{z}{\reserveagentm}\geq  \utilagent(\valagent)+\equivcumulative{\agent}{z}{}\geq \tfrac{e-1}{e}v_iz.
\end{equation}

	The lemma then follows from noting that $\vvalagent(\valagent)\leq \valagent$, and hence when $\vvalagent(\valagent)\geq 0$, the inequality in (\ref{eq:genvvalcover}) is a weakening of that in (\ref{eq:genvvalcoverres}).
\end{proof}

The following theorem then follows from Lemma~\ref{lem:genrevtradeoff} exactly as Theorem~\ref{thm:bnerev} follows from Lemma~\ref{lem:revtradeoff}.

\begin{theorem}
	In mechanisms that exclude agents below the monopoly reserves $\reservesm$, the resolution of generalized revenue covering for Bayes-Nash equilibrium and the objective of revenue is at most $2e/(e-1)$.
\end{theorem}


==> rc-bne.tex <==
\subsection{Incomplete Information}
\label{sec:bne}

%strategies, interim allocations
%agent normal-form

==> rc-single.tex <==
\subsection{Single-Item Auctions}
\label{sec:rc-single}

The simplest winner-pays-bid mechanism is the single-item first price auction. Each agent submits a bid $\bidagent$, and the highest bidder wins. In this mechanism, the relationship between an agent's competition and the revenue is one-to-one; each agent's threshold bid is the bid of another agent.

\begin{theorem}
	The single-item first-price auction has revenue covering approximation $1$.
\end{theorem}

\begin{proof}
	The revenue of a first-price auction under bid profile $\bids$ is the highest bid, $\max_\agent \bidagent$. Each agent's threshold bid $\thresholdagent(\bidothers)$ is the bid of some agent, and not necessarily the maximum. Any feasible allocation $\allocalt$ satisfies $\sum_{\agent}\allocaltagent\leq 1$. These three facts immediately imply the desired inequality: $\rev(\mech,\bids)\geq\sum\nolimits_{\agent}\thresholdagent(\bidothers)\allocaltagent.$
\end{proof}
By Lemmas \ref{lem:dettoexp1} and~\ref{lem:dettoexp2}, the single-item first-price auction also has expected revenue covering approximation $1$ with any reserves.

==> welfare-bne.tex <==
\subsection{Incomplete Information}
\label{sec:bne}

%strategies, interim allocations

==> welfare-bneallpay.tex <==
\subsubsection{All-Pay Mechanisms}
\label{sec:welfare-bneallpay}

For all-pay mechanisms, we consider only randomized allocation rules. Pure approximate Nash equilibria do not exist, rendering an analysis of deterministic mechanisms unnecessary.

\begin{lemma}\label{lem:aptradeoff}
	The individual efficiency of exact best response in all-pay mechanisms with randomized allocation rules is $\eta=1/2$.
\end{lemma}
\begin{proof}
	To lower bound the \vc, note that the agent selects their best response bid $\bid$ to maximize their utility $\bidutil(\bid)=\val\bidallocation(\bid)-\bid$. For any allocation probability $\allocation\in[0,1]$, agent $\agent$ could choose to get allocation probability at least $\allocation$ by bidding their interim threshold $\interthresh{}{\allocation}$. Hence, $\bidutil(
	\bid(\val))\geq \val \allocation-\interthresh{}{\allocation}$ for all $\allocation\in[0,1]$. We may rearrange this as $\interthresh{}{\allocation}\geq \val\allocation-\bidutil(\bid(\val))$. Since we also have $\interthresh{}{\allocation}\geq 0$, we may write:
	\begin{align*}
		\cumuthreshagent{}{z}{}\geq \int_0^z \max(\val\allocation-\bidutil(\bid(\val)),0)\,d\allocation&=\int_{\bidutil(\bid(\val))/\val}^z \val\allocation-\bidutil(\bid(\val))\,d\allocation\\
		&=\tfrac{\val}{2}-\bidutil(\bid(\val))+\tfrac{\bidutil(\bid(\val))^2}{2\val}.
	\end{align*}
	We therefore have $\bidutil(\bid(\val))+\cumuthreshagent{}{z}{}\geq \val/2+\bidutil(\val)^2/2\val$. Holding $\val$ fixed and minimizing the righthand side as a function of $\bidutil(\bid(\val))$ yields a lower bound of $\val z/2$, as desired. To exhibit tightness, choose $\val=1$, $\bidallocation(\bid)=\bid$ for $\bid\in[0,1]$, and $\bid = 0$.
\end{proof}
